A shuffle algebra point of view on operator-valued probability theory

We extend the shuffle algebra perspective on scalar-valued non-commutative probability theory to the operator-valued case. Given an operator-valued probability space with an algebra $B$ acting on it (on the left and on the right), we associate operators in the operad of multilinear maps on $B$ to the operator-valued distribution and free cumulants of a random variable. These operators define a representation of a PROS of non-crossing partitions. Using concepts from higher category theory, specifically $2$-monoidal categories, we define a notion of unshuffle Hopf algebra on an underlying PROS. We introduce a PROS of words insertions and show that both the latter and the PROS of non-crossing partitions are unshuffle Hopf algebras (in a $2$-monoidal sense). The two relate by mean of a map of unshuffle bialgebras (in a $2$-monoidal sense) which we call the splitting map. Ultimately, we obtain a left half-shuffle fixed point equation corresponding to free moment-cumulant relations in a shuffle algebra of bicollection homomorphisms on the PROS of words insertions. Right half-shuffle and shuffle laws are interpreted in the framework of boolean and monotone non-commutative probability theory, respectively. Keywords: operator-valued non-commutative probability theory, higher category theory, duoidal categories, operads, properads, PROS, shuffle algebra, half-shuffles

==> notation.tex <==
\newcommand{\freeunitary}{{U^{\langle n \rangle}}}
\newcommand{\mfreeunitary}{{\lmss{U}^{\langle n \rangle}}}
\newcommand{\genfree}{L_{n}}

\newcommand{\unitaryfd}{U^{\mathbb{K}}_{n,d}}
\newcommand{\unitaryfdr}{U^{\mathbb{R}}_{n,d}}
\newcommand{\unitaryfdc}{U^{\mathbb{C}}_{n,d}}
\newcommand{\unitaryfdh}{U^{\mathbb{H}}_{n,d}}
\newcommand{\munitaryfd}{\lmss{U}_{N}^{\mathbb{K}}}
\newcommand{\munitaryfdr}{\lmss{U}_{N}^{\mathbb{R}}}
\newcommand{\munitaryfdc}{\lmss{U}_{N}^{\mathbb{C}}}
\newcommand{\munitaryfdh}{\lmss{U}_{N}^{\mathbb{H}}}
\newcommand{\re}{\mathrm{Re}}
\newcommand{\Real}{\lmss{Re}}
\newcommand{\Co}{\lmss{Co}}
\newcommand{\noisefd}{\lmss{W}_{N}}
\newcommand{\noisefree}{\lmss{W}}
\newcommand{\unitaryalg}{\mathcal{O}\langle nd\rangle}
\newcommand{\unitarygp}{U(N,\mathbb{K}}
\newcommand{\unitaryr}{U(N,\mathbb{R}}
\newcommand{\unitaryc}{U(N,\mathbb{C}}
\newcommand{\unitaryh}{U(N,\mathbb{H}}
\newcommand{\hermitianalg}{\mathcal{H}\langle n \rangle}
\newcommand{\hermitianalgc}{\mathcal{H}\langle n \rangle}
\newcommand{\udualgroup}{\mathcal{O}\langle n \rangle}
\newcommand{\GLR}[1]{\mathrm{G}\mathrm{L}_{#1}(\mathbb{R})}
\newcommand{\GLC}[1]{\mathrm{G}\mathrm{L}_{#1}(\mathbb{C})}

%% BRAUER

\newcommand{\transpo}{\lmss{T}_{k}}
\newcommand{\projector}{\lmss{W}_{k}}
\newcommand{\tr}{\lmss{T}_{k}}
\newcommand{\pr}{\lmss{W}_{k}}
\newcommand{\trd}{\lmss{T}_{k,\lmss{d}}}
\newcommand{\prd}{\lmss{W}_{k,\lmss{d}}}

\newcommand{\trnm}{\lmss{T}_{k,n}}
\newcommand{\prnm}{\lmss{W}_{k,n}}

\newcommand{\trexc}{\lmss{T}^{\neq}_{k}}
\newcommand{\prexc}{\lmss{W}^{\neq}_{k}}
\newcommand{\trexcd}{\lmss{T}^{\neq}_{k,\lmss{d}}}
\newcommand{\prexcd}{\lmss{W}^{\neq}_{k,\lmss{d}}}

\newcommand{\trpd}[1]{\lmss{T}^{+}_{k,\lmss{d}}(#1)}
\newcommand{\prpd}[1]{\lmss{W}^{+}_{k,\lmss{d}}(#1)}

\newcommand{\trp}[1]{\lmss{T}^{+}_{k}(#1)}
\newcommand{\prp}[1]{\lmss{W}^{+}_{k}(#1)}
\newcommand{\trpnc}[1]{\lmss{T}^{+,\scalebox{0.6}{$\bullet$}}_{k}(#1)}
\newcommand{\prpnc}[1]{\lmss{W}^{+,\scalebox{0.6}{$\bullet$}}_{k}(#1)}

\newcommand{\trpnm}[1]{\lmss{T}^{+}_{k,n}(#1)}
\newcommand{\prpnm}[1]{\lmss{W}^{+}_{k,n}(#1)}

\newcommand{\brauer}{{\mathcal{B}_{k}}}
\newcommand{\brauerdf}[1]{\mathcal{B}_{k}^{#1}}

\newcommand{\Brauer}{{\mathcal{B}_{k}}}
\newcommand{\cbrauer}{\overset{\circ}{\mathcal{B}}_{k}}
\newcommand{\cbrauerd}{\overset{\circ}{\brauerd}}
\newcommand{\cbrauerf}[1]{\overset{\circ}{\mathcal{B}^{#1}_{k}}}
\newcommand{\vbrauer}{\mathbb{C}\left[\mathcal{B}_{k}\right] }
\newcommand{\brauerz}{\mathcal{B}^{{ \scalebox{0.6}{$\bullet$}}}_{k}}
\newcommand{\ncc}[1]{{#1}^{\scalebox{0.6}{$\bullet$}}}
\newcommand{\nccc}[1]{#1^{\scalebox{0.6}{$\bullet$}}}

\newcommand{\brauergen}{(\ncc{b},c_{b})}
\newcommand{\Twist}{\lmss{Tw}^{\scalebox{0.6}{$\bullet$}}}
\newcommand{\genbrauerz}{(\ncc{b},c_{b})}
\newcommand{\brauerd}{\mathcal{B}_{k}^{\lmss{d}}}
\newcommand{\brauernm}{\mathcal{B}_{k,n}}
\newcommand{\trdiag}{{\lmss{T}_{k}^{=}}}
\newcommand{\prdiag}{{\lmss{W}_{k}^{=}}}
\newcommand{\trdiagd}{{\lmss{T}_{k,\lmss{d}}^{=}}}
\newcommand{\prdiagd}{{\lmss{W}_{k,\lmss{d}}^{=}}}

\newcommand{\trexcp}[1]{
\ensuremath{\lmss{T}_{k}^{{\neq},+}(#1)}}
\newcommand{\prexcp}[1]{
\ensuremath{\lmss{W}_{k}^{{\neq},+}(#1)}}

\newcommand{\trdiagp}[1]{
\ensuremath{\lmss{T}_{k}^{{=},+}(#1)}}
\newcommand{\prdiagp}[1]{
\ensuremath{\lmss{W}_{k}^{{=},+}(#1)}}

\newcommand{\trdiags}[1]{\lmss{T}_{k}^{=,s}(#1)}
\newcommand{\prdiags}[1]{\lmss{W}_{k}^{=,s}(#1)}
\newcommand{\trexcs}[1]{\lmss{T}_{k}^{\neq,s}(#1)}
\newcommand{\prexcs}[1]{\lmss{W}_{k}^{\neq,s}(#1)}
%% Rectangular

\newcommand{\cluster}{{\mathcal{C}\mathcal{R}\mathcal{O}\langle\lmss{d}\rangle}}
\newcommand{\runitaryalg}{\mathcal{R}\mathcal{O}\langle n \rangle}
\newcommand{\rdunitaryfd}{U^{\mathbb{K}}_{\{\lmss{d}\}}}
\newcommand{\runitaryfd}{U^{\mathbb{K}}_{\lmss{d}}}
\newcommand{\rdunitaryfdN}{U^{\mathbb{K}}_{\{d_{N}\}}}
\newcommand{\runitaryfdN}{U^{\mathbb{K}}_{d_{N}}}
\newcommand{\runitaryfdNr}{U^{\mathbb{R}}_{d_{N}}}
\newcommand{\runitaryfdNc}{U^{\mathbb{C}}_{d_{N}}}
\newcommand{\runitaryfdNh}{U^{\mathbb{H}}_{d_{N}}}

%%Rectangular

\newcommand{\rpseudounitary}{\mathcal{R}\pseudounitary}
\newcommand{\rpseudoorthogonal}{\mathcal{R}\mathcal{O}(-+)}


%% Split pseudounitary
%%PSEUDO

\newcommand{\pseudounitarygp}{\mathbb{U}(p,q,\mathbb{K})}
\newcommand{\pseudorealgp}{O(p,q)}
\newcommand{\pseudocompgp}{U(p,q)}
\newcommand{\pseudoquatgp}{Sp(p,q)}

\newcommand{\grpuk}[2]{\mathrm{U}(#1,#2,\mathbb{K})}
\newcommand{\grpur}[2]{\mathrm{U}(#1,#2,\mathbb{R})}
\newcommand{\grpuc}[2]{\mathrm{U}(#1,#2,\mathbb{C})}
\newcommand{\grpuh}[2]{\mathrm{U}(#1,#2,\mathbb{H})}

\newcommand{\pseudounitary}{\mathcal{U}(-,+)}
\newcommand{\pseudounitaryh}{\mathcal{U}^{h}(-,+)}

\newcommand{\pseudoorthogonal}{\mathcal{O}(-,+)}
\newcommand{\pseudohermitian}{\mathfrak{h}(-,+)}
\newcommand{\pseudohermitianfs}{\mathfrak{h}(-,+)\left[\left[h\right]\right]}
\newcommand{\pseudohermitianfsd}{\mathcal{M}_{2}\left(\pseudohermitianfs\right)}
\newcommand{\pseudosymmetricfd}{\lmss{W}^{p,q}_{\mathbb{R}}}
\newcommand{\pseudohermitianfd}{\lmss{W}^{p,q}_{\mathbb{C}}}
\newcommand{\pseudosymplecticfd}{\lmss{W}^{p,q}_{\mathbb{H}}}

\newcommand{\pseudounitaryfd}{\Lambda^{p,q}_{\mathbb{C}}}
\newcommand{\pseudoorthogonalfd}{\Lambda^{p,q}_{\mathbb{R}}}
\newcommand{\pseudoorthosympfd}{\Lambda^{p,q}_{\mathbb{H}}}
\newcommand{\pseudounitarykfd}{\Lambda^{p,q}_{\mathbb{K}}}
\newcommand{\spseudounitaryfd}{\Lambda^{p,p}_{\mathbb{C}}}
\newcommand{\spseudoorthogonalfd}{\Lambda^{p,p}_{\mathbb{R}}}
\newcommand{\spseudoorthosympfd}{\Lambda^{p,p}_{\mathbb{H}}}

\newcommand{\pseudounitaryrvfd}{V_{p}^{\mathbb{K}}}
\newcommand{\pseudounitaryrvfdpq}{V_{p,q}^{\mathbb{K}}}
\newcommand{\pseudohermitianrvfd}{W_{p}^{\mathbb{K}}}
\newcommand{\sproc}{{\Lambda_{\mathbb{K}}^{p,p}}}
\newcommand{\condexp}{E^{p,q}_{\mathbb{K}}(t)}
%%

%% FREE LIMITING PROCESS
\newcommand{\dnoise}{W}
\newcommand{\mdnoise}{\lmss{W}}
\newcommand{\freerv}{V}
\newcommand{\mfreerv}{\lmss{V}}
\newcommand{\matrixdnoise}{\begin{bmatrix} \mfreerv(t)_{++} & \mfreerv(t)_{-,+}\\ \mfreerv(t)_{+-} & \mfreerv(t)_{--} \end{bmatrix}}
\newcommand{\trmatrixdnoise}{\begin{bmatrix} \mfreerv_{++}(t)^{\star^{\prime}} & \mfreerv_{-+}(t)^{\star^{\prime}} \\ \mfreerv_{-+}(t)^{\star^{\prime}} & \mfreerv_{--}(t)^{\star^{\prime}}\end{bmatrix}}
\newcommand{\gen}{\mathcal{L}}
\newcommand{\genpph}{\mathcal{G}}

%%Matrices
\newcommand{\mmptranspo}{\lmss{T}^{-,+}}
\newcommand{\mpmtranspo}{\lmss{T}^{+,-}}
\newcommand{\mmmtranspo}{\lmss{T}^{-,-}}
\newcommand{\mpptranspo}{\lmss{T}^{+,+}}

\newcommand{\mmpprojector}{\lmss{W}^{-,+}}
\newcommand{\mpmprojector}{\lmss{W}^{+,-}}
\newcommand{\mmmprojector}{\lmss{W}^{-,-}}
\newcommand{\mppprojector}{\lmss{W}^{+,+}}
\newcommand{\genph}{\begin{bmatrix*}[l]h_{+} & h_{+-}^{\star} \\ h_{+,-} & h_{-}\end{bmatrix*}}
\newcommand{\casimirr}{\lmss{C}_{p,q}^{\mathbb{R}}}
\newcommand{\casimirh}{\lmss{C}_{p,q}^{\mathbb{H}}}
\newcommand{\casimirczero}{\overset{00}{\lmss{C}_{p,q}^{\mathbb{C}}}}
\newcommand{\casimircun}{\overset{01}{\lmss{C}_{p,q}^{\mathbb{C}}}}
\newcommand{\casimirk}{\lmss{C}_{p,q}^{\mathbb{K}}}
\newcommand{\casimirkp}{\lmss{C}_{p}^{\mathbb{K}}}

%%Split Proc


%%diffusion speeds
\newcommand{\diffp}{v}
\newcommand{\diffc}{c}

%% Twist operators
\newcommand{\twist}{\lmss{Tw}^{\scalebox{0.6}{$\bullet$}}}

%%fluctuations
\newcommand{\braueri}{\mathcal{B}_{\infty}}
\newcommand{\brauerir}{\mathcal{B}_{k,\text{irr}}}
\newcommand{\braueriir}{\mathcal{B}_{\infty,\text{irr}}}

\newcommand{\statek}{\mathcal{B}^{\mathbb{K}}}
\newcommand{\statei}{\statek_{\infty}}
\newcommand{\stateiir}{\statek_{\text{irr}, \infty}}

\newcommand{\fock}{\mathcal{F}\left[\braueri^{\mathbb{K}} \right]}
\newcommand{\fockirr}{\mathcal{F}\left[\stateiir\right]}

\newcommand{\tensor}{T\left[\braueri^{\mathbb{K}} \right]}


\newcommand{\tbraueri}{\tilde{\mathcal{B}}_{\infty}}
\newcommand{\tfock}{\mathcal{F}\left[\statek\right]}
\newcommand{\fockone}{\mathcal{F}(\mathcal{B}_{\infty}^{\mathrm{irr}})}
\newcommand{\tensors}{T\left[\statek \right]}
\newcommand{\tensorsirr}{T\left[\statek\right]}
\newcommand{\ttensors}{T\left[\statek \right]}
\newcommand{\stater}{\mathcal{B}^{\mathbb{R}}}
\newcommand{\statec}{\mathcal{B}^{\mathbb{C}}}

\newcommand{\staterirr}{\mathcal{B}^{\mathbb{R},\mathrm{irr}}}
\newcommand{\statecirr}{\mathcal{B}^{\mathbb{C},\mathrm{irr}}}
\newcommand{\statekirr}{\mathcal{B}^{\mathbb{K},\mathrm{irr}}}
\renewcommand{\labelitemi}{$\scriptstyle \bullet$}


\def\Alg{{\rm Alg}}
\def\biMod{{\rm biMod}}

\def\rCoMod{{\rm rCoMod}}
\def\lCoMod{{\rm lCoMod}}
\def\coModAlg{{\rm coModAlg}}
\def\freem{\mathrel{\dot\sqcup}}
\def\free{\mathrel{\sqcup}}

\def\Hom{{\rm Hom}}
\def\id{{\rm id}}
\def\Prob{{\rm Prob}}

\def\path{{\sf P}}
\def\seqloop{{\mathcal{P}\left(\lmss{L}_{\textrm{Aff},0}\left(\mathbb{R}^{2}\right)\right)}}
\def\seqlasso{{\overset{\circ}{\mathcal{P}}(\lmss{lassos})}}

%% Category

\def\isom{{\overset{\cong}{\to}}}
\def\Obj{{\mathrm{Obj}}}
\def\Vect{{\mathrm{Vect}}}

%% Misc
\def\C{{\mathbb C}}
\def\R{{\mathbb R}}
\def\H{{\sf H}}
\def\F{{\mathcal{F}}}
\def\U{{\mathbb{U}}}
\def\K{{\mathbb{K}}}
\def\bcyan{{\color{cyan} \scalebox{0.8}{$\bullet$}}}
\def\bmage{{\color{magenta} \scalebox{0.8}{$\bullet$}}}
\def\boran{{\color{orange} \scalebox{0.8}{$\bullet$}}}

